Offline Reinforcement Learning from Images with Latent Space Models

Offline reinforcement learning (RL) refers to the problem of learning policies from a static dataset of environment interactions. Offline RL enables extensive use and re-use of historical datasets, while also alleviating safety concerns associated with online exploration, thereby expanding the real-world applicability of RL. Most prior work in offline RL has focused on tasks with compact state representations. However, the ability to learn directly from rich observation spaces like images is critical for real-world applications such as robotics. In this work, we build on recent advances in model-based algorithms for offline RL, and extend them to high-dimensional visual observation spaces. Model-based offline RL algorithms have achieved state of the art results in state based tasks and have strong theoretical guarantees. However, they rely crucially on the ability to quantify uncertainty in the model predictions, which is particularly challenging with image observations. To overcome this challenge, we propose to learn a latent-state dynamics model, and represent the uncertainty in the latent space. Our approach is both tractable in practice and corresponds to maximizing a lower bound of the ELBO in the unknown POMDP. In experiments on a range of challenging image-based locomotion and manipulation tasks, we find that our algorithm significantly outperforms previous offline model-free RL methods as well as state-of-the-art online visual model-based RL methods. Moreover, we also find that our approach excels on an image-based drawer closing task on a real robot using a pre-existing dataset. All results including videos can be found online at https://sites.google.com/view/lompo/ .

==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Deep reinforcement learning (RL) has shown successes in game playing such as Atari~\citep{mnih2013playing}, Minecraft~\citep{oh2016control}, and Go~\citep{silver2017mastering}, and control problems such as simulation locomotion~\citep{kenneally2016design}
%%CF.10.27: maybe cite a real locomotion paper instead, e.g. the SAC algorithms and applications paper had a minitaur locomotion task I think.
%%KY.11.7: addressed
%%CF.11.8: It still says simulated locomotion... Whenever you address a comment, you should be rereading the entire part of that text (in this case, the entire first sentence)
and real-world robotic manipulation~\citep{levine2016end, zeng2018learning, kalashnikov2018qt}. However, deep RL algorithms are generally not yet practical for real-world systems due to several challenges. First, deep RL methods require a large amount of online trial-and-error to learn a skill, which is too expensive to be realized in the real world. Second, the online interactions with the environment could be unsafe in the real world since the robot could damage infrastructure or even hurt people when it hasn't yet mastered the skill. In the meantime, it is generally much easier to collect large diverse datasets that consists of videos of the real-world applications before the start of the RL procedure. Offline RL methods that learn policies from those fixed datasets can immediately resolve the aforementioned challenges while still attaining good performance. However, it is also difficult to apply existing offline RL methods to real robot learning problems because robots typically only have access to raw sensor inputs, which prior offline RL methods struggle to handle as shown in Figure X. \todo{add comparisons between CQL from states and CQL from images.} Thus, these offline RL methods have thus far fallen short of their potential of scaling to real robotics problems.
%%CF.10.27: I think this sentence above is a bit weird for a couple reasons -- there are some successes with high dimensional inputs and we aren't going to be doing things outside of a lab environment. To avoid this awkwardness, I would suggest starting by motivating offline RL, and then from there, saying that it's difficult to apply these offline RL methods to real robot learning problems because robots typically only have access to raw sensor inputs, which prior methods struggle to handle. i.e. these offline RL methods have thus far fallen short of their potential of scaling to real robotics problems. [this ending would rely on having real robot results though.]
%%KY.11.7: I rewrite the above paragraph based on the suggestion.
%%CF.7.7: This isn't specific to pixel inputs, which is a bit weird since you started this list by saying that there are several challenges with addressing high-dimensional inputs. To avoid this awkwardness, I might start out by start out by talking about how there have been successes in deep RL, but is generally not yet practical for real-world systems, and then discuss what's missing to make it practical, i.e. the ability to leverage offline data and scale to high-dimensional observation spaces.
%%KY.9.11: I rewrote the above sentences.
% Finally, it is also challenging to learn a compact representation that captures the underlying information of the task and enables efficient reinforcement learning.
%%CF.7.7: I might not mention the compact representation part until a bit later. It's a core aspect of the method, but I don't think that it's a critical part of the problem that we're trying to solve. I would also be happy if we had a great approach that didn't learn a compact latent space.
Therefore, designing offline RL algorithms that can learn meaningful representations from the pre-recorded visual datasets and achieve efficient policy learning from such representations would make offline RL more practical for tackling real-world problems.

%%CF.10.27: this discussion of prior work seems much more long-winded than it needs to be. You have an entire related work section to discuss these sorts of things.
%%CF.11.8: This paragraph is still much longer than it needs to be. I think you can cut down the discussion of model-free methods.
Prior works in offline RL have shown promising performances in low-dimensional observation spaces.  Offline model-free methods identify that the major challenge of offline RL methods is the large extrapolation error of the Q-function when evaluated on out-of-distribution actions~\citep{fujimoto2018off} and address this issue
% by regularizing the learned policy to the behavioral policy induced by the static dataset~\cite{fujimoto2018off, kumar2019stabilizing, wu2019behavior, jaques2019way, peng2019advantage, siegel2020keep, wang2020critic, nachum2019algaedice} or learning lower bound Q functions to avoid overestimation when encountering out-of-distribution actions~\cite{kumar2020conservative}.
by regularizing the Q function~\citep{kumar2020conservative} or the learned policy~\citep{fujimoto2018off, kumar2019stabilizing, wu2019behavior, jaques2019way, peng2019advantage, siegel2020keep, wang2020critic, nachum2019algaedice}.
%%CF.7.7: I think the above sentence goes into a bit more detail than what's necessary.
%%KY.9.11: I shortened it a bit.
Recent advances on offline model-based RL methods~\citep{kidambi2020morel, yu2020mopo, matsushima2020deployment} further improve the performance of these methods by expanding the offline dataset with model rollouts and penalizing out-of-distribution states based on model uncertainty.
% taking care of both out-of-distribution actions and \emph{states} through uncertainty quantification of the learned model.
%%CF.7.7: I would shorten the last part of the above sentence. I suggested one way above.
%%KY.9.11: Is there a suggestion above? I shortened it a bit.
Despite those advantages, offline model-based RL methods have yet shown success in vision-based control domains.
Since offline model-based RL algorithms learn a policy and a model from an offline dataset, they pose a major difficulty that stems from the distributional shift between the states generated from the learned model and the learned policy and the offline data. To address such a difficulty, quantifying the uncertainty of the generated states becomes crucial to avoid the method from suffering extrapolation error.
Due to the reason above, directly applying current offline model-based RL algorithms to high-dimensional inputs is challenging, since learning a dynamics model from raw sensory inputs, i.e. a video prediction model~\citep{finn2017deep, ebert2018visual}, that also admits good uncertainty estimates, is notably difficult. For example, learning an ensemble of video prediction models, a common approach for uncertainty quantification, could be prohibitively expensive and inefficient. Hence, these methods cannot be readily applied to vision-based tasks. The core problem that this work is attempting to tackle is: can we design a new offline model-based RL algorithm that scales to visual inputs and handles uncertainty in high-dimensional observation spaces?
%%CF.10.27: I think this last part of the sentence should be obvious if you do a good job at making it clear why uncertainty estimation is at the core of offline RL. I also think that the problem we want to solve should be fairly clear by the end of the first paragraph. This is a bit late to be stating the problem, since the paragraph above should be making it clear why prior methods don't already solve the problem.
%%KY.11.7: I revised the above paragraph to point out the importance of uncertainty quantification. I also state the problem of applying offline RL to images in the previous paragraph, but here I want to state that we want to design an algorithm that can handle uncertainty in the image space, which is a bit more specific than the whole problem we want to solve.

%%CF.7.7: Generally, I think the above paragraph is great. Mostly wording feedback on the above

%%CF.7.7:  Maybe start with: "To address the challenge of acquiring uncertainty estimates, a key aspect of our approach is to represent model uncertainty within a lower-dimensional latent space. ..."
To address the challenge of acquiring uncertainty estimates, a key aspect of our approach is to represent model uncertainty within a lower-dimensional latent space. 
% Recent model-based RL works have shown great success in learning latent models for vision-based control tasks in \cite{Hafner2019PlanNet, Dreamer2020Hafner}.
%%CF.10.27: I might exclude this previous sentence. I don't think it adds much. (but definitely discuss these prior methods in the RW)
%%KY.11.7: addressed.
Specifically, we learn an ensemble of dynamics models in the latent space and use the disagreement of predictions across latent models in the ensemble for uncertainty quantification. Since the latent model is known to capture the compact representation of the true dynamics and the model ensemble has been used for estimating epistemic uncertainty, we expect that the ensemble of the latent models is able to capture the uncertainty of the true dynamics to some degree.
%%CF.10.27: I'm not sure I fully understand what you're trying to convey in this sentence? are you trying to convey that you can learn a probabilistic model in the latent space (e.g. with a Gaussian output)? 
%%KY.11.7: Sorry, missing the ensemble in the version before. Now fixed.
Moreover, since the latent representation is low-dimensional, learning the model ensemble in the latent space is also much more efficient than
%%CF.10.27: are you trying to capture the uncertainty with the model or with the ensemble or both? this part of the sentence suggests that it's just the ensembe and is a bit confusing when taking into account the previous sentence.
%%KY.11.7: I mean the ensemble. See the comment above.
than performing the same operation directly from images. Following \cite{yu2020mopo}, we construct an uncertainty-penalized MDP in the latent space with the disagreement among the latent models in the ensemble as the penalty for the reward in the constructed MDP and then optimize the policy under the uncertainty-penalized MDP. 
%%CF.7.7: Can you elaborate on the above a little bit more? Without making the connections to ensembles, the reader may not understand why it is efficient.
%%KY.9.11: Addressed.

%%CF.10.27: It would be good to have a teaser figure in the top left that illustrates the key idea and/or illustrates the problem setting and/or highlights some of the results.
\todo{add teaser.}

%%CF.7.7:  I might put a paragraph break here and start this by saying "The main contribution of this work is an algorithm, offline visual model-based reinforcement learning, which learns ..."
%%KY.9.11: addressed.
The main contribution of this work is an algorithm, LOMPO, which enables reinforcement learning of vision-based control policies from offline datasets.
%%CF.10.27: I might put part of this description at the end of the paragraph above, and maybe rephrase this sentence to something ilke "The main contribution of this work is an algorithm, Latent Offline Model-based Policy Optimization (LOMPO), which enables reinforcement learning of vision-based control policies from offline datasets.
%%KY.11.7: addressed.
%%CF.7.7: I would cut "following prior work~\cite{}" because it may make it come across as more incremental.
%%CF.7.7: In the below, I might delete the first sentence and rephrase the second sentence to: "We extend the theoretical results in \cite{} to show that <describe result in this paper>."
%%CF.7.7: My reasoning for the above is that the intro is really about this paper, and you can use the related work section to discuss the relation to prior work. It's not critical that they clearly understand the relation to prior work at the end of the intro.
%%KY.9.11: Sounds good. I revised the paragraph below.
%%CF.10.27:  Maybe rephrase the below to "By building on the results of Yu et al, we theoretically show that LOMPO ..." Referring to the algorithm by name will better connect it with the previous sentence.
%%KY.11.7: addressed.
By building on the results of \cite{yu2020mopo}, we theoretically show that optimizing a policy in the latent uncertainty-penalized MDP corresponds to maximizing a lower bound of the return of the policy in the high-dimensional observation space.
%%CF.10.27: The above is quite a mouthful. Can you break it up into two more digestible sentences? You could also just exclude the first part of the sentence, since I assume the second part is the main result?
%%KY.11.7: addressed.
Based on these theoretical findings, we train a policy under the latent uncertainty-penalized MDP with the reward penalized by the disagreement across predictions of latent models in an ensemble.
% %%CF.10.27: it's not especially clear how the below connects to the first phrase above.
% we train an ensemble of latent dynamics models and use the disagreement among the latent models in the ensemble as the reward penalty to upper bound the estimate of true model error.
% %%CF.10.27: maybe simply say "and use the disagreement among the latent models in the ensemble as an estimate of the true model error."
% Thus, this reward penalty can quantify the uncertainty of high-dimensional pixel inputs in a latent space, which mitigates the challenges of estimating uncertainty from images and makes offline RL feasible.
% %%CF.10.27: This seems a bit repetitive with the third paragraph.
We evaluate our algorithm on extensive simulated vision-based continuous control tasks and two real-world robotic manipulation tasks. We find that LOMPO learns the optimal behaviors on those challenging tasks while previous offline model-free RL algorithms and state-of-the-art online model-based RL methods failed to do so.
%%CF.10.27: I would spend a bit more time summarizing the results, and make more concrete statements about the improvement.
%%KY.11.7: I expanded it a bit but it will depend on the final results.

% Discuss deep RL in general. Mention that deep RL suffers from high sample complexity
% %%CF.8.30: See comment about sample complexity in the abstract
% and safety concerns, which makes it impractical to be applied in real-work settings. Thus learning from static datasets without interacting with the environment is pivotal to the progress of deep RL methods.
% %%CF.8.30: I think it would also be nice to emphasize/mention the challenge of vision & high-dimensional sensor observations in this first paragraph.

% Introduce offline RL and its challenges, i.e. large extrapolation error of the Q functions evaluated on out-of-distribution state and action pairs.
% %%CF.8.30: You'll need to be pretty careful about statements regarding OOD state and actions. Our method certainly doesn't work when you are not close to the training distribution.
% Discuss how prior model-free methods mitigate this issue by either regularizing the learned policy to stay close to the behavioral policy (cite BCQ, BEAR, BRAC, AWR, etc.) or learning lower bound Q functions to avoid overestimation when encountering out-of-distribution data (cite CQL). 
% %%CF.8.30: You can probably keep this explanation of prior model-free works very short. 
% Discuss how offline model-based RL methods enjoys a few advantages over model-free offline RL methods, e.g. generalization to OOD data (cite MOPO), minimax optimality (cite MOReL), and deployment-efficient (cite BREMEN). 
% %%CF.8.30: offline model-free methods are also deployment efficient, so this is not an advantage.
% Mention how prior offline MBRL handles distributional shift and model uncertainty. However, despite those advantages, offline model-based RL methods have yet shown success in vision-based control domains.
% %%CF.8.30: Can you discuss why it is challenging to directly apply them? One way to do this would be to discuss how learning a model of raw sensor observations that admits good uncertainty estimates is hard. For example, learning an ensemble of video prediction models may be prohibitively expensive. Hence, these methods cannot be readily applied to the vision-based setting.
% %%CF.8.30: May even be worth citing visual foresight here, since it is a vision-based algorithm that has been applied in the offline setting. I'm not sure about this though, because this paragraph will already have a lot of content and the reader is not likely to think immediately of visual foresight. (Good to bring up in the related work though)

% %%CF.8.30: When you introduce the algorithm, it would be good to tie it back to the challenges mentioned before, and make it clear how it addresses the challenges that make prior methods unfit for 
% Introduce our algorithm that combines offline MBRL with latent planning. Discuss how latent model-based RL works (cite PlaNet, Dreamer, etc). Discuss how uncertainty estimation is done in the latent dynamics model. Summarize our experimental results.
% %%CF.8.30: I would probably summarize the experimental results at the end of the last paragraph rather than at the end of this paragraph.

% Summarize the main contributions of our paper. 1) First offline MBRL algorithm.
% %%CF.8.30: It's not the first offline MBRL algorithm. MOReL and MOPO were that. :)
% %%CF.8.30: I would probably summarize the main contribution as "an offline model-based RL algorithm that scales to high-dimensional observations." And important secondary contributions being the theoretical guarantees and the empirical study of its performance.
% 2) Proposes a new method (with theoretical guarantees) that handles uncertainty and distributional shifts with visual observations. 3) Works well in extensive image-based control tasks.

==> method_mdp.tex <==
\newcommand{\D}{{\mathcal{D}}}
\newcommand{\Denv}{{\mathcal{D}_\text{env}}}
\newcommand{\Dmodel}{{\mathcal{D}_\text{model}}}
\newcommand{\given}{\,|\,}
\newcommand{\pib}{\pi^{\textup{B}}}

\section{Offline Model-based Policy Optimization in High Dimensions}
\label{sec:lompo}

\subsection{Problem Settings}
\label{sec:problem_setting}

\noindent \paragraph{Markov Decision Processes in Stateful High-Dimensional Space} We consider a class of MDPs that live in a high dimensional stateful observation space and supported by a compact latent state representation. Concretely, we consider MDPs of the form: $M = (\mathcal{O}, \mathcal{A}, F, E, D, T, r, q_0, \gamma)$, where $\mathcal{O}$ denotes the the visual observation space and $\mathcal{A}$ the action space. The transition dynamics in image space is described by $F(o'|o,a)$, which is supported by a latent state representation: 
\[
F(o'|o, a) = \sum_{s'} D(o'|s') T(s'|E(o), a).
\]
Here, $E(o)$ is the encoding of the image into a latent state, $T(s'|s,a)$ denotes the transition dynamics in the latent space, and $D(\cdot|s)$ is a observation decoding distribution.\footnote{Note that for simplicity, we have used a summation over $s'$. In practice, the latent state representation and latent transition dynamics will be continuous.}
$r(o) \equiv r(E(o))$ denotes the reward function, $q_0(o)$ the initial observation distribution, and $\gamma \in (0, 1)$ the discount factor. Note that we have assumed a stateful high-dimensional observation space, which can often be realized by stacking multiple image frames~\citep{mnih2013playing}. Similar settings and assumptions have been considered in a number of prior works, either explicitly or implicitly~\aravind{cite a bunch of papers on pixel based control without recurrence}. The goal in reinforcement learning is to learn a policy $\pi(a|o)$ that maximizes the expected discounted return $\eta_M \coloneqq \mathbb{E}[\sum_{t=0}^\infty \gamma^tr(o_t, a_t)]$.

\noindent \paragraph{Offline Reinforcement Learning} is the setting where an agent has to learn the control policy using only a fixed dataset of interactions. In our work, we focus on offline RL in high-dimensional MDPs, where the agent has access to the fixed dataset $\Denv = {(o, a, r, o')}$. The dataset can be collected by a single or a mixture of behavior policies $\pib$. No additional interactions with the environment are possible. We call the distribution induced by $\Denv$ as the \textit{behavioral distribution}.

\noindent \paragraph{Model-Based Offline RL.} Model-based RL~\citep{suttonBook, sutton1991dyna} refers to a class of approaches for reinforcement learning, where an approximate model of the environment (dynamics and the reward) is learned and subsequently used for policy learning~\citep{sutton1991dyna, janner2019trust, RajeswaranGameMBRL} or model-based planning~\aravind{MPPI, PDDM etc}. A large body of work exists in model-based RL~(MBRL), some of which is summarized in Section~\ref{sec:related_work}. 

Early explorations with standard MBRL algorithms for offline RL yielded largely negative results~\cite{RossB12}. Recently, model-based RL in conjunction with the key idea of pessimism or conservatism, has emerged as a promising paradigm for offline RL~\citep{kidambi2020morel, yu2020mopo, matsushima2020deployment, argenson2020model}. Conservative versions of model-based RL have been shown to be minimax optimal and have also obtained state of the art results in many benchmark tasks. In this work, we build on the MOPO framework. Given a dataset $\Denv$ from an MDP $M$, MOPO learns an uncertainty penalized MDP with learned transition dynamics $\hat{T}(\cdot|s,a)$ and reward $\tilde{r}(s, a) = \hat{r}(s, a) - u(s, a)$ where $\hat{r}$ is the learned reward function and $u$ is an admissible uncertainty estimator such as $u(s,a) \geq \frac{r_{\max}}{1-\gamma} D_{TV}(T(s,a), \hat{T}(s,a))$.

A direct application of MOPO to high-dimensional MDPs would require learning the dynamics $\hat{F}(o'|o,a)$ and perform uncertainty quantification. Due to the high dimensionality, directly parameterizing and learning the dynamics model in the visual space can be extremely challenging. The need to perform uncertainty quantification over this high dimensional observation space further exacerbates the difficulty.

\noindent \paragraph{Latent Space Dynamics Modeling} To overcome the challenges associated with model learning and uncertainty quantification in visual observation spaces, we use latent space dynamics models. Inspired by recent advances in MBRL from pixels~\citep{Hafner2019PlanNet, Dreamer2020Hafner}, we learn a latent-space dynamics model with the following components:
\begin{gather}
\begin{aligned}
&\text{Image encoder:} &&s_t=E_\theta(o_t) \\
&\text{Latent transition model:} && T_\theta(s_{t+1}| s_t, a_t)\\
&\text{Reward predictor:} && R_\theta(r_t|s_t, a_t) \\
&\text{Image decoder:} && D_\theta(o_t|s_t).
\label{eq:latent_model}
\end{aligned}
\end{gather}%
Note that we use the subscript to denote parameterized functions that we wish to learn, with $\theta$ together representing the parameters of all the components in the model. We represent the image encoder and decoder using convolutional neural networks (CNNs). The transition model is implemented with a shared recurrent state space model (RSSM)~\citep{Dreamer2020Hafner} following prior work, but for simplicity of presentation, we interpret it as a multi layer perception.

The main advantage of a latent space model is the ability to simulate trajectories directly in the latent space without the need for image generation. This greatly enhances the memory and computational efficiency, enabling the generation of a large number of trajectories for policy learning in the latent space. The learned policy in the latent space can be composed with the learned encoder to obtain an observation-based policy.

To train the model, first consider a transiton in the dataset: $(o, a, o')$. Under our model, the likelihood of the transition is:
\[
\log \hat{F}(o'|o,a) = \log \left( \sum_{s'} D_\theta(o'|s') T_\theta(s'|s=E_\theta(o), a) \right).
\]
Directly optimizing the likelihood is intractable due to the required marginalization over all possible states. Instead, we train the latent space model by optimizing the evidence lowerbound (ELBO)~\citep{Blei2016VariationalIA}. Using Jensen's inequality and importance sampling, likelihood of the transition can be bounded as:
\begin{align}
\log \hat{F}(o'|o,a) & = \log \left( \sum_{s'} D_\theta(o'|s') T_\theta(s'|E_\theta(o), a) \right) \\
& \geq \sum_{s'} T_\theta(s'|E_\theta(o), a) \log D_\theta(o'|s') \\
& \geq \underbrace{\mathbb{E}_{q} \left[ \log D_\theta(o'|s') \right]}_{\mathrm{reconstruction}} - \underbrace{D_{KL} \left( q_\phi (s'|E_\theta(o),a), T_\theta(s'|E_\theta(o),a) \right)}_{\mathrm{consistency}}.
\end{align}
Here, we have introduced a variational distribution $q_\phi(\cdot|s,a)$ parameterized by $\phi$. It describes a next latent state distribution conditioned on the current latent state and action. In practice, we formulate both $q_\phi$ and $T_\theta$ as diagonal Gaussian distributions where the network parameterizes the mean of the Gaussian. The diagonal covariance of the Gaussian is also learned. We optimize the bound over both $\theta$ and $\phi$, in order to get a tight approximation. The gradient of the first term (reconstruction) is computed using the reparameterization trick, which allows for computing gradients with respect to both $\theta$ and $\phi$. To compute the gradient of the second consistency term, we use the knowledge that both $q_\phi$ and $T_\theta$ are diagonal Gaussian distributions, allowing us to form an analytical expression for the KL divergence. This analytical expression can be easily differentiated using automatic differentiation packages (e.g. pytorch). Overall, we solve the following optimization.
\begin{equation}
    \label{eq:elbo}
    \max_{\theta, \phi} \mathcal{L}(\theta, \phi) := \mathbb{E}_{\sim \Denv}
    \left[
    E_{q} \left[ \log D_\theta(o'|s') \right] - D_{KL} \left( q_\phi (s'|E_\theta(o),a), T_\theta(s'|E_\theta(o),a) \right)
    \right]
\end{equation}
For simplicity, we have only presented the learning of the dynamics model. The reward model is jointly learned along with the above loss function.

\subsection{Uncertainty Quantification in Latent Space Models} 
\label{sec:uq}

The goal of our method is to design an offline model-based RL method that handles high-dimensional inputs. Since we need to learn a model from the fixed dataset without further interaction with the environment, the model prediction will become less trustworthy as the model rollouts move further from the behavioral distribution. Such inaccurate model predictions would generate states that could negatively impact the policy optimization. Therefore, quantifying the uncertainty of the states generated by the learned model is important for offline model-based RL to avoid large extrapolation error on out-of-distribution states. However, estimating the model uncertainty in the high-dimensional observation space is challenging as the common approach in uncertainty quantification such as learning an ensemble of models is very memory-intensive and time-consuming when applied to visual dynamics models.

In this subsection, we present our offline visual model-based RL algorithm that address the above challenges by learning a latent dynamics model and estimating the model uncertainty in the compact latent space. Specifically, we first define the MDP in the latent space that exactly corresponds to the MDP in the stateful high-dimensional observation space defined in Section~\ref{sec:problem_setting}. Second, based on the latent MDP, we construct a latent uncertainty-penalized MDP where the reward is penalized by the uncertainty of the latent dynamics mode and show that the return of a constructed latent uncertainty-penalized MDP can be bounded from low by the return of the MDP in the latent space. Finally, we optimize the policy in the latent uncertainty-penalized MDP by maximizing the lower bound of the true return.

In order to quantify the uncertainty in the latent state space, we need to construct a new MDP in the latent space and connect such an MDP to the MDP in the stateful observation space. 
To this end, similar to \cite{cui2020control}, we first denote the MDP in the stateful observation space defined in Section~\ref{sec:problem_setting} as $\Mobs$ and then define a latent MDP $\Mstate$ induced by $\Mobs$ as $\Mstate = (\mathcal{S}, \mathcal{A}, T, r, \mu_0, \gamma)$ where $\mathcal{S}$ is the latent space, $T(s'|s, a)$ is the transition , and $\mu_0$ is the initial latent state distribution, which equivalent to the following generative process $o_0 \sim q_0(o), s_0 \sim E(s_0|o_0)$. Note that we abuse the notation of $E$ here to denote the composition of the image encoder $E_\theta$ and the inference model $q_\theta$ in Equation~\ref{eq:latent_model}.Similarly, we define the estimated latent MDP $\hatMstate = (\mathcal{S}, \mathcal{A}, \hatT, \bar{r}, \mu_0, \gamma)$ where $\hatT(s'|s,a)$ denotes the learned latent dynamics model. The objective of our algorithm is to learn an optimal policy $\pi(a|s)$ in $\hatMstate$ that also maximizes expected return in $\Mstate$.

\aravind{We propose to model uncertainty in the latent space. This has the advantage of $\ldots$. Kevin, can you write this part}

\subsection{Practical Implemetation}

==> method_old.tex <==
\section{Latent Offline Model-based Policy Optimization}

% While offline model-based RL methods such as MOPO achieve impressive results from low-dimensional observation spaces, they haven't shown successes in visual domains where the inputs are pixels.
%%CF.10.27: I might put this sentence in the previous section rather than here, so that this paragraph can focus on our approach rather than its relation to prior methods.
%%KY.11.7: addressed.
The goal of our method is to design an offline model-based RL method that handles high-dimensional inputs. Since we need to learn a model from the fixed dataset without further interaction with the environment, the model prediction will become less trustworthy as the model rollouts move further from the behavioral distribution. Such inaccurate model predictions would generate states that could negatively impact the policy optimization. Therefore, quantifying the uncertainty of the states generated by the learned model is important for offline model-based RL to avoid large extrapolation error on out-of-distribution states. However, estimating the model uncertainty in the high-dimensional observation space is challenging as the common approach in uncertainty quantification such as learning an ensemble of models is very memory-intensive and time-consuming when applied to visual dynamics models.
%%CF.10.27: This sentence kinds of comes out of nowhere. Why is estimating uncertainty important? Would also be nice to not be _too_ repetitive with the intro while still motivating the work.
%%KY.11.7: I added the discussion.

In this section, we present our offline visual model-based RL algorithm that address the above challenges by learning a latent dynamics model and estimating the model uncertainty in the compact latent space. Specifically, we first define the MDP in the latent space that exactly corresponds to the MDP in the observation space and then show that the return of a constructed latent MDP with the reward penalized by the uncertainty of the latent dynamics model can be bounded from low by the return of the MDP in the latent space (Section~\ref{sec:quantify}). Second, we optimize the policy in the latent uncertainty-penalized MDP by maximizing the lower bound of the true return (Section~\ref{sec:quantify}). Finally, we discuss our overall algorithm LOMPO and its practical implementation details (Section~\ref{sec:practice}).
%%CF.10.27:  I only see two subsections?
%%KY.11.7: addressed.

\subsection{Quantifying model uncertainty and optimizing the policy in the latent space}
\label{sec:quantify}
%%CF.10.27: The  paragraphs below are a bit hard to follow. You're also doing a lot more than what the subsection title suggests. For the former, can you give a bit more top-down information on where you're going with the prose? For example, why are you introducing two MDPs? A top down overview of the method before this subsection could also help achieve this. For example, see the 2nd paragraph of section 4 in the MOPO paper.
%%KY.11.7: I added a top down overview of the method before this subsection.
% The goal of our work is to learn a latent dynamics model that can be used to efficiently perform $k$-step rollouts in the latent space when the observation space is high-dimensional.
%%CF.10.27: Well, this isn't the only goal of our work, and also not the main goal of our work. This sentence is misleading.
In order to quantify the uncertainty in the latent state space, we need to construct a new MDP in the latent space and connect such an MDP to the MDP in the observation space. 
Moreover, we want the latent dynamics model to be equipped with the following property: the expected return of a policy $\pi(a|s)$ conditioned the latent state $s$ under learned latent dynamics model is a lower bound of the expected return of the policy (after the image decoder $D$) under the true dynamics in the observation space. To this end, similar to \cite{cui2020control}, we first denote the MDP in the observation space defined in Section~\ref{sec:prelim} as $\Mobs$ and then
% \footnote{We can make this MDP Markovian by using repeated actions for each observation in the replay buffer as in \cite{mnih2013playing}.}
%%CF.10.27: By this footnote, do you mean frame stacking? I think you need to do more than just repeat actions? Also, it seems weird to put this as a footnote because the main text is technically incorrect without this modification to the decision process.
%%KY.11.7: addressed and moved this discussion to prelim.
define a latent MDP $\Mstate$ induced by $\Mobs$ as $\Mstate = (\mathcal{S}, \mathcal{A}, T, \bar{r}, \mu_0, \gamma)$ where $\mathcal{S}$ is the latent space, $T(s'|s, a)$ is equivalent to the generative process $o \sim D(o|s), o'\sim F(o'|o, a), s' \sim E(s'|o')$, $\bar{r}(s, a) = r(o, a)$ $\forall s \sim E(s|o)$, and $\mu_0$ is the initial latent state distribution, which equivalent to the following generative process $o_0 \sim q_0(o), s_0 \sim E(s_0|o_0)$. Note that we abuse the notation of $E$ here to denote the composition of the image encoder $E_\theta$ and the inference model $q_\theta$ in Equation~\ref{eq:latent_model}.
%%CF.10.27: Equation 1 shows D as producing a distribution, not a deterministic function.
%%KY.11.7: addressed.
Similarly, we define the estimated latent MDP $\hatMstate = (\mathcal{S}, \mathcal{A}, \hatT, \bar{r}, \mu_0, \gamma)$ where $\hatT(s'|s,a)$ denotes the learned latent dynamics model. The objective of our algorithm is to learn an optimal policy $\pi(a|s)$ in $\hatMstate$ that also maximizes expected return in $\Mstate$.

%%CF.10.27: This paragraph on notation breaks the flow a lot. Is there a way to introduce this notation earlier, e.g. in the preliminaries?
%%KY.11.7: I moved it to the prelim
% To make the above objective more succinct, we introduce some notations. We first define $\mathbb{P}^\pi_{\hatT,t}(s)$ as the probability of being in state $s$ at time step $t$ following $\pi$ and $\hatT$. We denote the discounted state-action distribution $\rho^\pi_{\hatT}(s,a) := \sum_{t=0}^\infty \gamma^t \mathbb{P}^\pi_{\hatT,t}(s)\pi(a \given s)$. Note that $\rho^\pi_{\hatT}$, as defined here, integrate to $\frac{1}{1 - \gamma}$ and thus is not a properly normalized probability distribution. We also define (improper since not normalized) expectations with respect to $\rho^\pi_{\hatT}$ with $\Ei$, as in $\eta_{\Mstate}(\pi) = \Ei_{\rho^\pi_{\hatT}}[\hat{r}(s,a)]$.

With the above definitions and notations introduced in Section~\ref{sec:prelim}, by the definition of $\Mstate$, we have 
\begin{align}
% \vspace{-1cm}
    \eta_{\Mstate}(\pi) = \eta_{\Mobs}(\pi\circ E) \text{ }\forall \pi(a|s)\label{eq:equivalence}
% \vspace{-1cm}
\end{align}
\todo{this can perhaps be a proposition.}
where $(\pi\circ E)(a|o) = \int_s\pi(a|s)E(s|o)ds$, which is the image of the policy $\pi(a|s)$ in the observation space. Equation~\ref{eq:equivalence} shows that the expected return of any policy under $\Mstate$ is the same as the expected return of the image of such a policy in the observation space under $\Mobs$. With this equivalence, we can substitute $\Mobs$ with $\Mstate$ and quantify the model uncertainty entirely in the latent space. We can state that the objective of our method is to find a lower bound of the expected return of a policy $\pi$ under the true latent dynamics $\Mstate$ and then maximize the resulting lower bound w.r.t. $\pi$. Next, we quantify how the error of the dynamics model in the latent MDP translates into the uncertainty over the total return.
%%CF.10.27: Maybe rephrase this sentence to "Next, we quantify how the error of the dynamics model in the latent MDP translates into the uncertainty over the total return. "
%%KY.11.7: Addressed.
% of the policy under latent MDP $\Mstate$ via the error of the latent dynamics $\hatT$. 
% We first state the following lemma (adapted from \cite{yu2020mopo}), which characterizes the difference of the total return of a policy under $\hatMstate$ and $\Mstate$.

%%CF.10.27: This lemma seems identical to the lemma in the MOPO paper? Am I missing a difference?
% \begin{lemma}[Telescoping lemma] Let $G^\pi_{\hatMstate}(s,a) := \Esub{s' \sim \hatT(s,a)}[V_{\Mstate}^\pi(s')] - \Esub{s' \sim E(F(D(s), a))}[V_{\Mstate}^\pi(s')]$.
% Then,
% \begin{align}
% \eta_{\hatMstate}(\pi) - \eta_{\Mstate}(\pi) = \gamma \Eisub{(s,a) \sim \rho^\pi_{\hatT}}\left[G^\pi_{\hatMstate}(s,a)\right]\label{eqn:12}
% \end{align}
% \end{lemma}
% \label{lem:1}
% \begin{proof}
% Since $E(F(D(s), a))$ is the true dynamics model of $\Mstate$ by definition, then we can get the above result by directly applying Lemma 4.1 in \cite{yu2020mopo}.
%%CF.10.27: As I mentioned before, you define p(o|s) and D(o|s) to be stochastic functions. You need to reconcile this with what's stated here. The true p(o|s) may discard information from s, and s may not be recoverable.
% \end{proof}

Now with Lemma 4.1~\cite{yu2020mopo} and the assumption that $V_{\Mstate}^\pi \in c\mathcal{F}$ for some scalar $c$ and a function class $\mathcal{F}$ as in \cite{yu2020mopo}, we have
\begin{align}
    \eta_{\Mstate}(\pi) &= \Eisub{(s,a) \sim \rho^\pi_{\hatT,\mu_0}}\left[r(s, a) - \gamma G^\pi_{\hatMstate}(s,a)\right]\\
    &\geq\Eisub{(s,a) \sim \rho^\pi_{\hatT,\mu_0}}\left[r(s, a) - \gamma|G^\pi_{\hatMstate}(s,a)|\right]\\
    &\geq\Eisub{(s,a) \sim \rho^\pi_{\hatT,\mu_0}}\left[r(s, a)\nonumber\right.\\
    &\left.- \gamma\sup_{f\in\mathcal{F}}\left|\Esub{s' \sim \hatT(s,a)}[f(s')] - \Esub{s' \sim T(s'|s,a)}[f(s')]\right|\right]\\
    &\coloneqq \Eisub{(s,a) \sim \rho^\pi_{\hatT,\mu_0}}\left[r(s, a)\right.\nonumber\\
    &\left.- \gamma c d_\mathcal{F}\left(\hatT(s,a), T(s'|s,a))\right)\right]
\end{align}
Then, following \cite{yu2020mopo}, we assume that there exists an admissible error estimator, $u(s, a)$, that satisfies $d_\mathcal{F}\left(\hatT(s,a), E(F(D(s), a))\right) \leq u(s, a)$ for all $s, a$. With this assumption, we can construct the \textit{uncertainty-penalized} latent MDP $\tildeMstate = (\mathcal{S}, \mathcal{A}, T, \tilde{r}, \mu_0, \gamma)$ where $\tilde{r}(s, a) = \bar{r}(s, a) - \lambda u(s,a)$ where $\lambda = \gamma c$.

Under the uncertainty-penalized latent MDP, we first define $\epsilon_u(\pi) = \Eisub{(s,a)\sim \rho^\pi_{\hatT,\mu_0}}[u(s,a)]$. Then we proceed to show that the total return of a policy $\pi$ under the uncertainty-penalized latent MDP is a lower bound of the the total return under the latent state MDP induced by the observation MDP and the gap between the learned policy under the uncertainty-penalized latent MDP and the optimal policy $\pi^*$ depends on the latent dynamics model error $\epsilon_u(\pi^*)$. Directly following Theorem 4.4 in \cite{yu2020mopo}, we can show the above claims as following:
\begin{align}
    &\eta_{\Mstate}(\pi) \geq \eta_{\tildeMstate}(\pi),\\
    &\eta_{\Mstate}(\hat{\pi}) \ge \sup_{\pi}\{\eta_{\Mstate}(\pi) - 2\lambda\epsilon_u(\pi)\}
\end{align}
%%CF.10.27: I think it would be worth giving these equations their own lines, since they are the main theoretical result?
%%KY.11.7: Addressed.
where $\hat{\pi}$ is the policy learned via maximizing the return under $\tildeMstate$. 
% These two equations can be interpreted as the follows:
% the total return of a policy $\pi$ under the uncertainty-penalized latent MDP is a lower bound of the the total return under the latent state MDP induced by the observation MDP and the gap between the learned policy under the uncertainty-penalized latent MDP and the optimal policy $\pi^*$ depends on the latent dynamics model error $\epsilon_u(\pi^*)$. 
%%CF.10.27: Explaining what something means after you state it is not a good writing practice, since it usually means that what you were explaining will not have been clear to the reader when they read it. (It's fine to elaborate on something afterward, but generally, it's good to guide the reader so that everything is clear when they read each sentence.
%%KY.11.7: I move these explanations above.
In practice, we do not have access to the uncertainty quantification oracle $u(s, a)$ that upper bounds the latent model error, and we estimate the uncertainty of the latent model using heuristics as discussed in Section~\ref{sec:practice}.

\subsection{Main Algorithm}
\label{sec:practice}

\begin{figure*}
    \centering
    \includegraphics[width = 0.75\textwidth]{LOMPOFig2.png}
    \caption{Variational model training and the single latent rollout step of LOMPO.}
    %%CF.10.27: A more descriptive caption would be helpful. What are the main things you want the reader to take away from the figure?
    %%CF.10.27: Do the reconstructions correspond to actual reconstructions from the model? It would be best if they did. Right now, it looks like you just copied the images?
    \label{fig:model}
\end{figure*}
%%CF.10.27: The proportions of the figure are a bit awkward for a two-column figure. Can you change it to make it wider? e.g. put the legend on the left or right side along with the text like "Model Inference". You could also 
% \todo{Rafael, can you address the comments about the figure here?}
%%RR.11.7: Do we need this to be a two column figure to begin with? There is not that much detail I think

We now present our practical LOMPO algorithm, outlined in Algorithm~\ref{alg:euclid} in Appendix~\ref{app:alg}, and visualize the whole training pipeline in Figure~\ref{fig:model}. We describe our model training and policy optimization procedures in the following paragraphs.

\textbf{Variational Model Training.} We train a variation model of the environment similar to \cite{Hafner2019PlanNet} with a joint set of forward dynamics models in the latent space. The training objective is as follows:
\begin{equation} \label{eq1}
\begin{split}
\ln p(o_{1:T}|a_{1:T}) & = \int\prod_{t=1}^TT(s_t|s_{t-1}, a_{t-1})p(o_t|s_t)ds_{1:T} \\
%  & \geq \sum_{t=1}^T\Big[\mathbb{E}_{q(s_t|o_{\leq t}, a_{\leq t})}[\ln p(o_t|s_t)]-\\
%  & \mathbb{E}_{q(s_{t-1}|o_{\leq t-1}, a_{\leq t-1})}D_{\text{KL}}[q(s_t|o_{\leq t}, a_{<t})||T_t(s_t|s_{t-1}, a_{t-1})]\Big]
 & \geq \sum_{t=1}^T\Big[\mathbb{E}_\phi[\ln p(o_t|s_t)]-\\
 & \mathbb{E}_{\phi}D_{\text{KL}}[\phi(s_t|o_{\leq t}, a_{<t})||T_t(s_t|s_{t-1}, a_{t-1})]\Big]
\end{split}
\end{equation}

Here we used the standard variational approach and introduce an inference distribution $\phi(s_t|o_{\leq t}, a_{<t})$. Unlike previous works, at each step we sample a forward transition model $T_t$ from a fixed set of $K$ ensembles $\{T_1, \ldots, T_K\}$. This procedure has two main advantages:
%%CF.10.27: Can you motivate your design decisions _before_ you state them?
% \todo{Rafael, can you address this?}
\begin{enumerate}
    \setlength\itemsep{0em}
    \item By randomly sampling forward models we can train a full ensemble without the need for any additional components on top of the regular variational model.
    \item It grounds all forward models and the inference model in the same latent space representation, which allows us to randomly sample models during rollouts.
\end{enumerate}


For modeling the inference model and the latent transition model as defined in Equation~\ref{eq:latent_model}, we deploy a version of the standard RSSM,
%%CF.10.27: RSSM and model are technically redundant. I would just use the term "recurrent model" to avoid the extra jargon.
%%KY.11.7: I removed "model" and leave RSSM here since we already defined it in the prelim.
as in \cite{Hafner2019PlanNet, Dreamer2020Hafner} which has shown good performance for applications using model rollouts. We adopt the latent space representation $s_t = [d_t, z_t]$,
%%CF.10.27: we represent the representation? :)
%%KY.11.7: addressed
which consists of a deterministic $d_t$ and a sampled stochastic representation $z_t$. With such a latent space representation, we use the following components for the RSSM:
%%CF.10.27: See comment above about "RSSM model"
%%KY.11.7: addressed.
\begin{gather}
\begin{aligned}
&\text{Deterministic State Model:} &&d_t = f_{\theta}(d_{t-1}, z_{t-1}, a_{t-1}) \\
&\text{Stochastic Inference Model:} &&z_t \sim q_\theta(z_t|h_t, o_t)\\
&\text{Ensemble of Transition Models:} &&z_t \sim T_{\theta_k}(z_t| d_t, z_{t-1}, a_{t-1})\\
\label{eq:rssm}
\end{aligned}
\end{gather}%
 where $h_t = E_\theta(o_t)$ as defined in Equation~\ref{eq:latent_model}. The deterministic representation is shared between the forward and inference models. All the forward models in the ensemble share the same deterministic representation but separate stochastic representations. With this definition, the inference distribution $\phi_\theta(s_t|o_t, a_{t-1})$ is a composition of the deterministic encoder $E_\theta(o_t)$, deterministic state model $f_\theta(d_{t-1}, z_{t-1}, a_{t-1})$ and the stochastic inference model $q_\theta(z_t|h_t,o_t)$.

\textbf{Model-based Policy Optimization.}
%%CF.10.27: I think that the model-free portion of this header is going to be confusing, especially because of the method name that says that policy optimization is model-based
%%KY.11.7: I changed it to model-based policy optimization.
%%CF.10.27: Motivate design choices before you state them
% \todo{Rafael, can you address this?}
We train a policy and a critic
%%CF.10.27: actor-critic policy? How about just a policy and a critic?
%%KY.11.7: addressed.
with components $\pi_{\phi}(a_t|s_t), Q_{\phi}(s_t, a_t)$ on top of the latent space representation similar to \cite{SLAC2020Lee}, however we deploy model inference for the actor as well as the critic. We maintain two replay buffers $\mathcal{B}_{real}$, $\mathcal{B}_{sample}$.
%%CF.10.27: Reference the notation introduced for the fixed offline dataset?
The real data replay buffer contains data sampled from the inference distribution $s_{1:T}\sim \phi_{\theta}(s_{1:T}|o_{1:T}, a_{1:T-1})$.
%%CF.10.27:  you said before that E was deterministic? Now it is stochastic?
%%KY.11.7: replaced E with $\phi$
The latent data buffer contains data from rolling-out the policy in the model latent space. During rollouts states are propagated by picking a representation from a random model. As discussed in Section~\ref{sec:quantify}, the final rewards for the rollout use ensemble estimates and the uncertainty penalty term and are computed as:
%%CF.10.27: why is this the reward? should connect back to the theory.
%%KY.11.7: addressed.
\begin{equation}\label{latentreward}
    \tilde{r}_t(s_t, a_{t-1}) = \frac{1}{K}\sum_{i=1}^K r_{\theta}(s_t^{(i)}, a_t) - \lambda u(s_t, a_t)
\end{equation}
%%CF.10.27: remove the space between the equation and the text. Otherwise, latex treats the spacing and indentation incorrectly.
%%KY.11.7: addressed.
where $s^{(i)}_t\sim T_{\theta_i}(s_{t-1}, a_{i-1})$ are sampled from each forward model and $s_t$ is sampled from $\{s^{(i)}_t, i=1,\ldots, K\}$. Here $u(s_t, a_t)$
%%CF.10.27: In section IV.A, the uncertainty estimator was u(s,a). why is it u(s_t, a_{t-1}) here?
%%KY.11.7: I believe it's an implementation detail. Removed this for now.
is an estimate of model uncertainty and $\lambda$ is a penalty parameter. In particular, we pick $u(s_t, a_t)$ as disagreement of the latent model predictions in the ensemble, i.e. the variance of log-likelihoods under the stochastic model ensemble
$$u(s_t, a_t) = \mathbf{Var}(\{\log T_{\theta_i}(s_t|s_{t-1}, a_{t-1}), i=1,\ldots, K\}),$$ 
since ensembles have been shown to capture the epistemic uncertainty~\citep{bickel1981some} and also work well for model-based RL in practice~\citep{yu2020mopo, kidambi2020morel}.
%%CF.10.27: I would cite MOPO here instead of Sekar. Sekar uses ensembles for a completely different purpose. MOPO is also arguably a more relevant citation than Chua and Rajeswaran as well, since it specifically uses the ensemble in order to be conservative
%%KY.11.7: addressed
Finally the actor and critic $\pi_{\phi}(a_t|s_t), Q_{\phi}(s_t, a_t)$ are trained using standard off-policy training algorithm using batches of equal data mixed from the real and sampled replay buffers. Similar to \cite{yu2020mopo} we find that maintaining a fixed sampling proportion is important in preventing distributional shift in the actor-critic training.

%%CF.10.27: Would be nice to have a somewhat concise algorithm box in the main text.
\todo{Add a concise algorithm box.}

==> prelim_mdp.tex <==
\iffalse

\newcommand{\D}{{\mathcal{D}}}
\newcommand{\Denv}{{\mathcal{D}_\text{env}}}
\newcommand{\Dmodel}{{\mathcal{D}_\text{model}}}
\newcommand{\given}{\,|\,}
\newcommand{\pib}{\pi^{\textup{B}}}


\section{Preliminaries}
\label{sec:prelim}

\noindent \paragraph{Markov Decision Processes in Stateful High-Dimensional Space} We consider a class of MDPs that live in a high dimensional stateful observation space and supported by a compact latent state representation. Concretely, we consider MDPs of the form: $M = (\mathcal{O}, \mathcal{A}, F, E, D, T, r, q_0, \gamma)$, where $\mathcal{O}$ denotes the the visual observation space and $\mathcal{A}$ the action space. The transition dynamics in image space is described by $F(o'|o,a)$ which is supported by a latent state representation: 
\[
F(o'|o, a) = \sum_{s'} D(o'|s') T(s'|E(o), a)
\]
where $E(o)$ is the encoding of the image into a latent state, $T(s'|s,a)$ denotes the transition dynamics in the latent space, and $D(\cdot|s)$ is a observation decoding distribution.\footnote{Note that for simplicity, we have used a summation over $s'$. In practice, the latent state representation and latent transition dynamics will be continuous.}
$r(o, a) \equiv r(E(o), a)$ denotes the reward function, $q_0(o)$ the initial observation distribution, and $\gamma \in (0, 1)$ the discount factor. Note that we have assumed a stateful high-dimensional observation space, which can often be realized through multiple image frames~\cite{mnih2013playing}. Similar settings and assumptions have been considered in a number of prior works, either explicitly or implicitly~\aravind{cite a bunch of papers on pixel based control without recurrence}. The goal in reinforcement learning is to learn a policy $\pi(a|o)$ that maximizes the expected discounted return $\eta_M \coloneqq \mathbb{E}[\sum_{t=0}^\infty \gamma^tr(o_t, a_t)]$.


% -----------------------------------

\noindent \paragraph{Model-based RL with latent dynamics} Our work takes a model-based approach~\citep{sutton1991dyna, watter2015embed} to solving high-dimensional MDPs. We first review prior work that learns latent space models for MDPs\footnote{We simplify presentation of prior work as applicable to our problem setting of interest described in Section~\ref{sec:prelim}}. Latent space dynamics models (see for example \citet{Hafner2019PlanNet, Dreamer2020Hafner}) typically have the following components:
\begin{gather}
\begin{aligned}
&\text{Image encoder:} &&s_t=E_\theta(o_t) \\
&\text{Inference model:} && q_\theta(s_t|s_{t-1}, a_{t-1}, h_t)\\
&\text{Latent transition model:} && \hatT_\theta(s_t| s_{t-1}, a_{t-1})\\
&\text{Reward predictor:} && p_\theta(r_t|s_t) \\
&\text{Image decoder:} && D_\theta(o_t|s_t).
\label{eq:latent_model}
\end{aligned}
\end{gather}%

The image encoder is represented as a convolutional neural network (CNN), while the inference model and the latent transition model are implemented as a shared recurrent state space model (RSSM)
%%CF.10.27:  I don't think this acronym has been defined. Maybe just say that it is a recurrent neural network for simplicity?
%%KY.11.7: addressed.
\cite{Hafner2019PlanNet}.
%%CF.10.27: This phrasing is weird. This section should _only_ be outlining things done by prior methods. I would probably just remove this sentence and the next ones, since it's easy to later say "Following~\citet{planet}, we parametrize the image encoder as ..." The prelim section generally _only_ needs to cover things that are important for being able to understand the methods section.
% The reward predictor and the image decoder are modeled as fully-connected neural networks and deconvolutional neural networks respectively and provide supervision signal to the latent dynamics. All the distributions are parameterized as diagonal Gaussians. We train all components jointly by maximizing a evidence lower bound (ELBO) similar to training a variational autoencoder (VAE)~\cite{kingma2013auto}.

Given a learned latent dynamics model, Dreamer~\citep{Dreamer2020Hafner} learns a policy (actor) $\pi_\phi(a_t|s_t)$ and a value function (critic) $V_\psi(s_t)$ in the latent space to achieve downstream tasks. The overall procedure is as follows. The latent dynamics model predicts a sequence of future latent spaces by first encoding the images sampled from a replay buffer and rolling out the latent transition model in the latent space. The value function attempts to predict the value of a latent state and the policy aims to maximize the predicted values by backpropagating the gradients through the latent dynamics model.
% Our method resembles Dreamer as we also use an actor-critic framework. However, instead of learning a value function, we adopt framework of SLAC~\cite{SLAC2020Lee}, where we learn a policy $\pi_\phi(a_t|s_t)$ and a Q function $Q_\psi(s_t, a_t)$ and maximize the maximum-entropy RL objective as in SLAC.
%%CF.10.27: I would probably leave out details about our method (and save it for the methods section). The most salient thing to mention here is that these prior methods cannot readily be applied to offline RL problems, and we will bridge this gap when we introduce our method in the next section.. 
%%KY.11.7: addressed/
% We will discuss more details in Section~\ref{sec:practice}.

%%CF.10.27: The below seems a bit disorganized. It would be nice to separate out any information on the problem statement and any important information on prior methods. Right now, the below mixes information from both of these.
\textbf{Offline model-based RL.} In our work, we focus on the setting of offline visual RL, where the agent only has access to a fixed dataset $\Denv = {(o, a, r, o')}$ collected by a single or a mixture of behavior policies $\pib$ without any interaction with the environment. We denote the distribution induced by $\Denv$ as the \textit{behavioral distribution}.

Our work builds on the broad notion and use of pessimism for offline learning~\citep{kidambi2020morel, yu2020mopo}. In particular, for our practical algorithm we build upon MOPO~\citep{yu2020mopo}, which tackles offline RL in the MDP $M = (\mathcal{S}, \mathcal{A}, T, r, \mu_0, \gamma)$ where $\mathcal{S}$ is the true low-dimensional state space and $\mu_0$ is the initial state distribution. MOPO trains an ensemble of probabilistic dynamics models and reward predictors $\{\hatT^i_\theta(s', r|s,a) = \mathcal{N}(\mu^i(s, a), \Sigma^i(s, a)\}_{i=1}^N$ parameterized by $\theta$ using data sampled from $\Denv$. During training, MOPO rolls out the learned dynamics model $\hatT_\theta(s'|s,a)$ for $k$ steps, and then penalize the reward of the state-action pairs generated by the model rollouts with an estimated model uncertainty as follows $$\tilde{r}(s, a) = r(s, a) - \lambda\max_{i=1,\dots, N}\|\Sigma_\theta^i(s, a)\|_\text{F}.$$ After applying the reward penalty, MOPO adds the generated data to a separate replay buffer $\Dmodel$ and updates the policy $\pi(a|s)$ with data sampled from $\Denv\cup\Dmodel$. MOPO theoretically shows that under the assumption that reward penalty term, which is implemented as the maximum variance across the ensemble in practice, is an admissible estimator of the true model error, optimizing a policy under the \textit{uncertainty-penalized} MDP $\tilde{M} = (\mathcal{S}, \mathcal{A}, \hatT, \tilde{r}, \mu_0, \gamma)$ is equivalent to optimize a lower bound of the return under the learned policy in the true MDP $M$. While MOPO achieve impressive results from low-dimensional observation spaces, they haven't shown successes in visual domains where the inputs are pixels. In the next section, we will extend MOPO to the setting with high-dimensional observations and we will show that an \textit{uncertainty-penalized} MDP in the latent space achieves the same effect.

\textbf{Notations.} In this paragraph, we introduce some notations. We first define $\mathbb{P}^\pi_{T,\mu,t}(s)$ as the probability of being in state $s$ at time step $t$ following $\pi$, $T$ and $\mu_0$. We denote the discounted state-action distribution $\rho^\pi_{T,\mu_0}(s,a) := \sum_{t=0}^\infty \gamma^t \mathbb{P}^\pi_{T, \mu, t}(s)\pi(a \given s)$. Note that $\rho^\pi_{T,\mu_0}$, as defined here, integrate to $\frac{1}{1 - \gamma}$ and thus is not a properly normalized probability distribution. We also define (improper since not normalized) expectations with respect to $\rho^\pi_{T,\mu_0}$ with $\Ei$, as in $\eta_{\Mstate}(\pi) = \Ei_{\rho^\pi_{T,\mu_0}}[r(s,a)]$.

\fi

==> related_work_old.tex <==
\section{Related Work}

%%CF.7.7: I would think about how you want to organize this section. The below paragraph covers both online model-based RL methods and offline model-free methods and offline model-based methods, which is a bit much. There are a couple ways that you could organize it, e.g. have one paragraph on offline RL methods and another paragraph about online model-based methods, or one paragraph on offline model-free and then a paragraph about offline model-based, and then a paragraph about online model-based. It's up to you, but it would be good to have some transitions between sections.
In the following section, we discuss prior works in offline model-free and model-based RL and offline model-based RL, while comparing them to our approach.

%%CF.10.27:  For paragraph headers, I would suggest including "\noindent" in front of all of them.
\textbf{Offline RL.} As discussed in Section~\ref{sec:intro}, online model-free RL methods suffer from high sample complexity and inability to scale to high-dimensional inputs.
%%CF.10.27: gap in the train of thought from the sentence above to the sentence below.
While off-policy algorithms~\citep{haarnoja2018soft, fujimoto2018addressing}
%%CF.10.27: maybe add some off-policy algorithms that have been demonstrated from images here?
can in principle apply to offline settings, they suffer from large extrapolation error of the Q functions on out-of-distribution actions and do not perform well in practice~\citep{fujimoto2018off}. 
%%CF.10.27: Should also cite somewhere: "Provably Good Batch Off-Policy Reinforcement Learning Without Great Exploration"
Offline model-free RL methods are designed to address this issue with three main categories: (1) regularizing the learned policy to be ``close`` to the behavioral policy~\citep{fujimoto2018off, kumar2019stabilizing, wu2019behavior, jaques2019way, nachum2019algaedice, peng2019advantage, siegel2020keep}, (2) estimating the uncertainty of the Q-function to determine how trustworthy the Q predictions are~\citep{agarwal2019striving, kumar2019stabilizing, wu2019behavior, levine2020offline},
%%CF.10.27: It seems strange to put the survey paper citation here?
and (3) learning a lower bound of the Q-function to avoid overestimation on out-of-distribution actions~\citep{kumar2020conservative}. Offline model-based RL methods have recently proposed to push the frontier of offline RL
%%CF.10.27: the above statement seems subjective and not really saying much of substance.
research and are shown to be minimax optimal for offline RL~\citep{kidambi2020morel}.
%%CF.10.27: This doesn't seem like the most salient thing to mention about offline MBRL methods. The generalization abilities seem to be more salient to me?
Prior works have been using models to optimize policies in a pessimistic~\citep{kidambi2020morel} or uncertainty-penalized~\citep{yu2020mopo} MDP with theoretical guarantees and outperform offline model-free methods in various continuous control settings. Offline model-based approaches have also been shown to be more deployment-efficient~\citep{matsushima2020deployment} and useful for planning and adapting to arbitrary goals~\citep{argenson2020model}.
%%CF.10.27: The above sort of comes across as an advertisement for offline MBRL methods, rather than a brief summary. :/ 
%%CF.10.27: There are also some other offline MBRL methods, e.g. there's an offline model-based planning paper from some folks at DeepMind. You could also look at what papers cite the MOPO and MORel papers.
However, all of these prior works focus on problems with low-dimensional state information. In contrast, we consider high-dimensional inputs, i.e. images, and aim to acquire complex skills directly from an offline visual datasets without ground-truth states. Our method builds upon \cite{yu2020mopo} and extends the uncertainty-penalized MDP framework to latent space by showing that the uncertainty in the latent space upper bounds the uncertainty in the high-dimensional observation space. Our latent dynamics model draws inspirations from prior works in online model-based RL, which we will discuss next. 

%%CF.10.27: All of the visual foresight works are examples of offline MBRL with visual inputs. Those are important to mention in the related work. (and maybe also compare to, actually)

\textbf{Online model-based RL.} Our work builds upon various prior works on online model-based RL with latent dynamics for image inputs. Prior works have learned dynamics models in a locally linear latent space to solve simulated tasks~\citep{watter2015embed, banijamali2018robust} and complex robotic tasks~\citep{zhang2019solar}.
%%CF.10.27: The DSAE paper also falls into this category above
\citep{Hafner2019PlanNet} trains a variational latent dynamics model and uses shooting-based methods for planning. Other works also utilize the variational latent dynamics model as a representation basis for a model-free policy \citep{Merlin2018Wayne,SLAC2020Lee,VRM2020Han}.
%%CF.10.27: add DeepMDP here?
The model closest to ours is \cite{Dreamer2020Hafner},
%%CF.10.27: I would try to avoid statements like the above, because they can mislead people into thinking that our work is very similar to Dreamer (especially for people that are just skimming and don't read the rest of this paragraph)
which trains a policy in the latent space by latent policy rollouts and directly differentiating through the latent dynamics. Different from \cite{Dreamer2020Hafner}, our model contains an ensemble of latent dynamics models and leverages the ensemble disagreement in the latent space for uncertainty quantification.
%%CF.10.27: Well, the most critical difference is that we are tackling a different problem setting. It is good to state the obvious for readers who aren't paying attention or aren't familiar with these prior works.
\cite{sekar2020planning} also trains an ensemble of latent dynamics, but uses the ensemble disagreement as an intrinsic reward to motivate exploration, which is contrary to our method that penalizes states generated by the latent model with high uncertainty.

% In order to facilitate learning in higher-dimensional spaces from fixed amounts of data we utilize recent developments in variational model-based reinforcement learning. There have been several related works beginning with \cite{Hafner2019PlanNet}, which trains a variational environment model and uses shooting-based methods for planning. Several other works utilize the variational model as a representation basis for a model-free policy, such as \cite{Merlin2018Wayne}, \cite{SLAC2020Lee} and \cite{VRM2020Han}. The model closest to ours is \cite{Dreamer2020Hafner}, which trains a policy in the latent space by latent policy rollouts and directly differentiating through the model dynamics. In contrast to our work all of these models are designed for the online reinforcement learning setup. There has also been significant recent interest in the offline-reinforcement learning setting with recent works such as (cite BCQ, BEAR,BRAC, AWR, etc.). The main approach of the model-free offline reinforcement learning literature has been do decrease the reliance on out-of distribution estimates by constraining either the policy to remain close to the data-generating policy or bounding the value function estimates. However, we found such methods tend to perform poorly in tasks with limited data and high-dimensional observations (remains to be seen), likely due to limited amount of supervision. In contrast offline-model based methods, such as \cite{yu2020mopo} (MBRL, Bremen and cite others) aim to learn a model of the environment and extend the data support by sampling additional data from the learned model. These approaches usually address model-uncertainty be deploying Bayesian methods or model ensembles. The work most similar to ours is \cite{yu2020mopo},
% %%CF.7.7: be careful with statements like "most similar to ours". It tends to invite criticism about this work not being novel enough. In many ways, MOPO is very different because it tackles a completely different problem.
% however unlike our proposed approach it focuses on low-dimensional ground-truth observations. Operating on high-dimensional observations, such as images in a low-data environment introduces significant additional difficulties, which we aim to address in this work.
